Mixing, tunnelling and the direction of time in the context of Reichenbach's principles

This work reviews the understanding of the direction of time introduced by Hans Reichenbach, including the fundamental relation of the perceived flow of time to the second law of thermodynamics (i.e. the Boltzmann time hypothesis), and the principle of parallelism of entropy increase. An example of a mixing process with quantum effects, which is advanced here in conjunction with Reichenbach's ideas, indicates the existence of a presently unknown mechanism that reflects global conditions prevailing in the universe and enacts the direction of time locally (i.e. the "time primer"). The possibility of experimental detection of the time primer is also discussed: if the time primer is CPT-invariant, its detection may be possible in high-energy experiments under the current level of technology.

==> figs.tex <==

\begin{figure}[h]
\begin{center}
\includegraphics[width=12cm,page=1,trim=0cm 5.5cm 0cm 6.8cm, clip ]{figst}
\caption{Footprints on a beach: a) effect of the second law of thermodynamics and b) effect of random disturbances. Curves: 1-realistic; 2-violating the second law; 3,3'- realistic disturbed by wind.}
\label{fig1}
\end{center}
\end{figure}

\bigskip
\bigskip
\bigskip
\bigskip
\bigskip
\bigskip
\bigskip
\bigskip


\begin{figure}[h]
\begin{center}
\includegraphics[width=6cm,page=2,trim=7cm 2.5cm 9cm 15cm, clip ]{figst}
\caption{Chemical reations shown in the form of casual forks.}
\label{fig2}
\end{center}
\end{figure}

\begin{figure}[h]
\begin{center}
\includegraphics[width=12cm,page=3,trim=1.5cm 2.2cm 0.2cm 4cm, clip ]{figst}
\caption{Experiment with admixture passing through semi-permeable membrane. Curves:  
1 -- position of the piston $x_m(t)$; 2 -- equilibrium $N_B(t)$; 3 -- $N_B(t)$ for $C=+1$; 4 -- $N_B(t)$ for $C=-1$. }
\label{fig3}
\end{center}
\end{figure}

\begin{figure}[h]
\begin{center}
\includegraphics[width=12cm,page=4,trim=1.2cm 3cm 2.2cm 7cm, clip ]{figst}
\caption{Tunnelling of a particle through the membrane: left -- with decoherence, right -- with recoherence, middle -- the membrane potential $U=U(x)$}
\label{fig4}
\end{center}
\end{figure}



%\begin{figure}[h]
%\begin{center}
%\includegraphics[width=10cm,page=5,trim=2cm 4cm 5cm 4cm, clip ]{figst}
%\caption{Influence of randomness on the choice between setting the initial or final conditions.}
%\label{fig5}
%\end{center}
%\end{figure}

\begin{figure}[h]
\begin{center}
\includegraphics[width=16cm,page=9,trim=0cm 0cm 0cm 0cm, clip ]{figst}
\caption{Circular arguments commonly used in explaining antecedent causality and the second law of thermodynamics.}
\label{fig6}
\end{center}
\end{figure}
